Template-Based Conjecturing for Automated Induction in Isabelle/HOL

Proof by induction plays a central role in formal verification. However, its automation remains as a formidable challenge in Computer Science. To solve inductive problems, human engineers often have to provide auxiliary lemmas manually. We automate this laborious process with template-based conjecturing, a novel approach to generate auxiliary lemmas and use them to prove final goals. Our evaluation shows that our working prototype, TBC, achieved 40 percentage point improvement of success rates for problems at intermediate difficulty level.

==> table.tex <==
Table \ref{table:tip} shows the characteristics of the problem sets we used for our evaluation.

\begin{center}
\begin{table}[ht!]
\begin{tabular}{|m{1.5cm}|m{2.5cm}|m{3.5cm}|m{4.5cm}|  }
 \hline
 \multicolumn{4}{|c|}{TIP} \\
 \hline
  & \hspace{1em} Isaplanner &  \hspace{1em} Prod & \hspace{1em} TIP15\\
 \hline
 data type & natural number, pair, list & natural number, pair list, boolean &  binary numbers, integers, list, regular expressions, trees\\
  \hline
functions & add, min, max, zip, sorts & add, multiply, reverse, sort, elem, union, intersection & ``weird'' add and multiple, sorts, trees, less than, power\\
 \hline
\end{tabular}
\caption{\text{Characteristics of each problem set.}}
\label{table:tip}
\end{table}
\end{center}
